Streaming Transformer Transducer Based Speech Recognition Using Non-Causal Convolution

This paper improves the streaming transformer transducer for speech recognition by using non-causal convolution. Many works apply the causal convolution to improve streaming transformer ignoring the lookahead context. We propose to use non-causal convolution to process the center block and lookahead context separately. This method leverages the lookahead context in convolution and maintains similar training and decoding efficiency. Given the similar latency, using the non-causal convolution with lookahead context gives better accuracy than causal convolution, especially for open-domain dictation scenarios. Besides, this paper applies talking-head attention and a novel history context compression scheme to further improve the performance. The talking-head attention improves the multi-head self-attention by transferring information among different heads. The history context compression method introduces more extended history context compactly. On our in-house data, the proposed methods improve a small Emformer baseline with lookahead context by relative WERR 5.1\%, 14.5\%, 8.4\% on open-domain dictation, assistant general scenarios, and assistant calling scenarios, respectively.

==> tex/old/exp-old.tex <==
\section{Experiments}
\label{sec:pagestyle}

\subsection{Data}
Our training data is a large-scale speech recognition dataset composed of two scenarios. The \textit{assistant} scenario consists of three parts. One is 13K hours of recordings collected from third-party vendors via crowd-sourced volunteers responding to artificial prompts with mobile devices. The content varies from voice assistant commands to a simulation of conversations between people. The second one is 1.3K hours of voice commands from production. The last one is 4K hours of speech for calling names and phone numbers generated by an in-house TTS model. The \textit{open domain} dictation has 18K hours of human transcribed data from public video and 2M hours of public, unlabeled videos transcribed by a high-quality in-house model.

In evaluation, we use \textit{assi}, \textit{call} and \textit{dict} dataset. The \textit{assi} and \textit{call} is 13.6K manually transcribed de-identified utterances from in-house volunteer employees, which begin with a wake word. The \textit{dict} is 8 hours open domain dictation from crowd-sourced workers recorded via mobile devices.

All datasets are de-identified with no personally identifiable information (PII). The data was further augmented with various distortion methods: speed perturbation~\cite{ko2015audio}, simulated reverberation SpecAugment \cite{park2019specaugment}, and randomly sampled additive background noise extracted from public videos.

\subsection{Experiment Setting}
We use 80-dimensional log Mel filter bank features at a 10ms frame rate in all the experiments. We experiment with two sizes of transducer models, 32M parameter and 73M parameters. In 73M parameter models, \emph{SpecAugment} \cite{park2019specaugment} without time warping and dropout 0.1 are used. We found that the 32M parameter models are underfitting a large amount of training data. The best performance is obtained by not using dropout and \emph{SpecAugment}.

For both 32M and 73M models, we use a 640-dimensional superframe concatenation of 8 consistent frames with a downsampling factor of 8 to 73Ms frame rate. In the 32M model, the superframe is projected to a 256-dimensional vector for 18 Emformer layers with convolution layers and a 320-dimensional vector for 21 Emformer layers without convolution layers. In the 73M model, the superframe is mapped to a 512-dimensional vector for  20 layers Emformer without convolution layers and a 384-dimensional vector for 20 layers Emformer with convolution layers. The 32M models use four heads for self-attention. The 73M models use eight heads for self-attention. In all the experiments, we use kernel size 7 for depth-wise convolution operations. The left context sizes are 2.4 s and 800 ms for the 73M and 32M model, respectively.

The 73M model uses a predictor that consists of a 256-dimensional embedding layer with 4096 sentence pieces~\cite{kudo2018sentencepiece}, three LSTM layers with 512 hidden nodes, and a linear projection layer with 1024 output nodes. The 32M model reduce the number of LSTM layer to 1. In all the experiments, alignment restrict RNNT~\cite{jay_2020_arrnnt} is used. we use the adam optimizer~\cite{kingma2014adam} with warming-up and the learning rate 1e-3. The training of all the models uses 32 Nvidia V100 GPUs. We evaluate the models by word error rate (WER) for accuracy and the real-time factors (RTFs) and speech engine perceived latency (SPL) for latency. The SPL measures the time from the speech engine gets the last word from user utterance to the speech engine transcribes the last word and gets the endpoint signals.

On the 32M model, 

\subsection{Improvement from non-causal convolution}
Table.~\ref{tab:32m_noncausal} gives the WER, RTF and SPL results for models with 32M parameters and 73M parameters. The results show that by keeping the overall context size (the sum of block size and lookahead context size) the same, using lookahead context gives WER improvement over not using lookahead context especially for open domain dictation scenarios. The results also show that using convolution and macaron structure improves the baseline when both baseline and treatment use the same context information. The direct application of causal convolution doesn't improve the baseline model which leverages the lookahead context. Comparing row 4 with row 3, row 8 with row 7 in Table.~\ref{tab:32m_noncausal}, using causal convolution performs worse than baseline with lookahead context.

Using lookahead context adds more computation for encoders in transducer model, as the forward logic has duplicated computation for the lookahead context. For the 73M model, row 7 and row 9 show $10\%$ relative RTF increase. However, using lookahead context provides accurate ASR results which yields slightly better speech perceived latency (SPL).


\begin{table}[htbp]
    \centering
    \caption{WER, RTF and SPL impact from non-causal convolution and lookahead context.Column '#p' gives the number of parameters in each model. Column 'w/C' denotes whether the convolution is applied or not. `C` and 'R' represents the block size and lookahead context size. The unit for `C`, `R` and `SPL` is millisecond.}
    \begin{tabular}{|cccc|ccc|cc|}
    \hline
   \#p & w/C &C &R&\textit{dict} & \textit{ass} & \textit{call} & SPL &RTF\\
   \hline
    32M &N & 400 & 0 & 18.31& 5.17 & 6.57 &635 &0.21\\
    32M &N & 320 & 80 & 17.09 & 5.05 & 6.68 &588 &0.22\\
    \hline
    32M& Y & 400 & 0 &17.70  &4.78  &6.76  &626 &0.22\\
    32M&Y & 320 & 80 & 17.02 & 4.66 & 6.53 &605 &0.22\\
    \hline
     73M& N & 400 & 0 & 16.78 & 4.18 & 6.19 &606 &0.27\\
    73M&N & 320 & 80 & 15.49 & 3.98 & 5.81 &599 &0.30\\
    \hline
    73M&Y & 400 & 0 &16.11  &4.05  &5.94  &615 &0.27\\
    73M&Y & 320 & 80 & 14.67 & 3.65 & 5.85 &595 &0.30\\
    \hline 
    \end{tabular}
    \label{tab:32m_noncausal}
\end{table}

\subsection{Improvement from talking heads attention}
Table.~\ref{tab:th} shows the impact of applying talking heads attention on top of Emformer with non-causal convolutions. For 32M small models, the talking heads attention generates $4.6\%$, $3.8\%$ and $2.8\%$ relative WERR on open-domain dictation, assistant general queries and assistant calling queries. For the 73M models, the talking heads attention gives similar results as the baseline model. We believe that the small 32M model doesn't have enough modeling capacity to learn well for the large amount of training data. The introduction of talking heads attention improves the small model's learning capacity. 

\begin{table}[htbp]
    \centering
    \caption{WER, RTF and SPL impact from talking heads attention. Column 'w/TH' denotes whether the talking heads attention is applied or not.
    %The unit for `SPL` is millisecond.
    }
    \begin{tabular}{|cc|ccc|cc|}
    \hline
    \# params &w/TH&\textit{dict} & \textit{ass} & \textit{call} & SPL &RTF\\
    \hline
    % 32M & N & 16.80 & 4.48 & 6.58 &516 &0.22\\
    % report chkp4
    \multirow{2}{*}{32M} & N &  17.02 & 4.66 & 6.53 &605 &0.22\\
     & Y & 16.25 &  4.48 &  6.35 &620  &0.23\\
    \hline
    % 73M & N & 14.67 & 3.657 & 5.85 &541 &0.30\\
    % report ckp4
    \multirow{2}{*}{73M} & N & 14.67 & 3.65 & 5.85 &595 &0.30\\
     & Y & 14.69  & 3.64 & 5.79 &574 & 0.30[\
    \hline 
    \end{tabular}
    \label{tab:th}
\end{table}

\subsection{Improvement from the context compression}

The impact of context compression is reported in Table~\ref{tab:contextcomp}.
For 32M small models,
using 2 slots of context compression
outperforms the baseline only with regular left context by
$3.2\%$, $5.7\%$, $5.5\%$
on 
open-domain dictation, assistant general, and assistant calling test sets.
Besides,
there is some level of complementarity between the talking-head attention and context compression schemes. By combining both methods, the word error rate can be further improved while maintaining similar SPL and RTF as the baseline.
\begin{table}[htbp]
    \centering
    \caption{WER and RTF and SPL impact from the context compression. Column `L' stands for the length of left context. Column `CL' stands for the length of compressed left context. The unit of both columns is slot: for `L', 1 slot means 100ms; for `CL', 1 slot implies 400ms, i.e. block size. 
    %Column 'w/TH' denotes talking head attention.
    }
    \begin{tabular}{|cccc|ccc|cc|}  
    \hline
    \#p & L & CL & w/TH &\textit{dict} & \textit{ass} & \textit{call} & SPL & RTF\\ 
    \hline
     & 10 & 0 & N & 17.02 & 4.66 & 6.53 & 605 & 0.22\\
    32M & 8 & 2 & N & 16.48 &  4.39 & 6.17 & 597 & 0.24 \\
     & 8 & 2 & Y & 16.22 & 4.32 & 6.12 & 589 & 0.24 \\
    \hline
      & 30 & 0 & N & 14.67 & 3.65 & 5.85 & 595 &0.30 \\
    78M  & 8 & 2 & N & 14.67 & 3.74 & 5.95 & 559 & 0.29 \\
      & 8 & 2 & Y& 14.69 & 3.66 & 5.77 & 554 & 0.29 \\
    \hline   
    \end{tabular}
    \label{tab:contextcomp}
\end{table}


==> tex/old/intro-old.tex <==
\section{Introduction}
\label{sec:format}
Nowadays, streaming automatic speech recognition (ASR) systems equip many embedded devices like mobile phones, speakers, and smartwatches.  On-device ASR  has the advantage of eliminating the audio and results transferring between devices and a server, which serves the users with fast, reliable, and privacy-preserving speech recognition experiences.

Sequence transducer networks~\cite{Graves2012,he2019rnnt} are widely used for on-device automatic speech recognition due to their superior performance and compactness. A sequence transducer model has an encoder to capture the context information from acoustic signals, a predictor to model the grammar, syntactic and semantic information, and a joiner to combine the two parts. The work~\cite{zhang_2020,Yeh_2019} showed replacing the LSTM encoder with the self-attention-based transformer~\cite{vaswani2017} yielded the state-of-the-art of accuracy on public benchmark datasets, which is consistent to the trend in applying transformer in various scenarios for automatic speech recognition~\cite{dong2018speech,karita2019comparative,sperber2018self,zhou2018syllable,chengyi_wang_2020,frank_zhang_2020,povey2018time,yongqiang_2019_icassp,emformer,conformer,Chunyang_2020_interspeech,cfyeh_asru_2020}. 

There are a wide range of .
One popular variant of transformer models in speech recognition tasks is Conformer~\cite{conformer}, which adds the depth separable convolutions and macaron network structure~\cite{macaron_2019} into the transformer. The work~\cite{xie_2021_streaming_transformer,jiahui_2021_fastemit} simplified the depth-wise convolution in conformer to causal convolution to support streaming scenarios.
In~\cite{cfyeh_asru_2020} the non-causal convolution is used to support streaming speech recognition. However, they have to use sequential block processing to avoid training and decoding inconsistency. The sequential block processing segments the input sequences into multiple blocks and sequentially do the model training on each block. The sequential block process is slow in training for low latency scenarios and incapable of industry application. In this work, we successfully make the non-causal convolution possible for parallel block processing, giving a similar training speed to Emformer model training.


% However, causal convolution uses the history context information in s self-attention while ignoring the lookahead context. 
% In this paper, we leverage a similar architecture as conformer but uses non-causal convolution to support streaming. Experiments on a large scale of industry data show that given the same amount of context information, using segment size 320 ms and lookahead context 80ms gives significant accuracy improvement over only using 400 ms segment without lookahead context. 
% In this work, we successfully make the non-causal convolution possible for parallel block processing, giving a similar training speed to Emformer model training.



In multi-head self-attention~\cite{vaswani2017}, the different heads conduct the attention computation separately. The attention outputs are concatenated at the end. Recently, the work~\cite{talking_heads_attention} proposed a Talking-Heads attention method to break the separation among different heads by inserting
two additional learned light weighed linear projections transferring information across different heads. Our experiments show that the application of this new variant of self-attention also gives more than $4.5\%$ WERR on an open-domain dictation scenario.

The Emformer~\cite{emformer} and the augmented memory transformer~\cite{Chunyang_2020_interspeech} supports streaming speech recognition by using block processing where the whole utterance is segmented into multiple blocks. The self-attention performs the computation on the current block and its surrounding left context and lookahead context. An augmented memory scheme is proposed to store the information from processed blocks,
which explicitly introduces compact long-form context while 
maintains limited computation and runtime memory consumption in inference.
The attention output from the mean of the current block is used as a memory slot for future blocks. 
In this work, we further simplify the memory extraction process similar to~\cite{compress_transformer}, referred to as context compression.
Rather than using the self-attention output from the mean of each block, we directly use the linear projection of each block as memory. The experiments show that this simplification further improves the accuracy.

==> tex/related_work.tex <==
\section{Related Word}
\label{sec:related_work}


